A Close Look at Deep Learning with Small Data

In this work, we perform a wide variety of experiments with different deep learning architectures on datasets of limited size. According to our study, we show that model complexity is a critical factor when only a few samples per class are available. Differently from the literature, we show that in some configurations, the state of the art can be improved using low complexity models. For instance, in problems with scarce training samples and without data augmentation, low-complexity convolutional neural networks perform comparably well or better than state-of-the-art architectures. Moreover, we show that even standard data augmentation can boost recognition performance by large margins. This result suggests the development of more complex data generation/augmentation pipelines for cases when data is limited. Finally, we show that dropout, a widely used regularization technique, maintains its role as a good regularizer even when data is scarce. Our findings are empirically validated on the sub-sampled versions of popular CIFAR-10, Fashion-MNIST and, SVHN benchmarks.

==> tables/models_structure.tex <==

\begin{tabular}{llllllllllllllllccc}
		\toprule

               & \multicolumn{15}{c}{\textbf{Model block}} & \multicolumn{3}{c}{\textbf{Trainable parameters }(M)}\\
		\midrule

               & \multicolumn{3}{c}{$f_{\phi}(\cdot)$} & \multicolumn{3}{c}{$f_{\theta}(\cdot)$} & \multicolumn{3}{c}{$f_{\gamma_{1}}(\cdot)$} & \multicolumn{3}{c}{$f_{\gamma_{2}}(\cdot)$} & \multicolumn{3}{c}{$f_{\gamma_{3}}(\cdot)$} & \multicolumn{1}{c}

{\multirow{2}{*}{CIFAR10}} & \multicolumn{1}{c}{\multirow{2}{*}{FMNIST}} & \multicolumn{1}{c}{\multirow{2}{*}{SVHN}} \\

\cmidrule(lr){2-4} 	\cmidrule(lr){5-7}  	\cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} 
\textbf{Model} & c1     & c2     & c3    & c1     & c2      & c3     & c1     & c2     & c3     & c1     & c2     & c3     & c1     & c2     & c3     & \multicolumn{1}{c}{} 

                        & \multicolumn{1}{c}{}                      & \multicolumn{1}{c}{}\\
		\midrule

CNN-lc         & --     & --     & --    & 20     & 30      & 50     & --     & --     & --     & --     & --     & --     & --     & --     & --     & 0.028                    

                        & 0.025                                         & 0.028                                           \\

CNN-mc         & --     & --     & --    & 40     & 60      & 100    & --     & --     & --     & --     & --     & --     & --     & --     & --     & 0.103                    

                        & 0.097                                         & 0.103                                           \\

CNN-hc         & --     & --     & --    & 80     & 120     & 200    & --     & --     & --     & --     & --     & --     & --     & --     & --     & 0.391                    

                        & 0.379                                         & 0.391                                           \\

SAE            & 20     & 40     & 50    & 50     & --      & --     & 40     & 20     & 3      & --     & --     & --     & --     & --     & --     & 0.095                    

                        & 0.091                                         & 0.095                                           \\

SASD-flip      & 20     & 40     & 50    & 50     & --      & --     & 20     & 10     & 3      & 20     & 10     & 3      & --     & --     & --     & 0.092                    

                        & 0.087                                         & 0.092                                           \\

SASD-rot       & 20     & 40     & 50    & 50     & --      & --     & 20     & 10     & 3      & 20     & 10     & 3      & 20     & 10     & 3      & 0.092                    

                        & 0.087                                          & 0.092                                           \\
\midrule

ResNet-20      &      &      &     &      &       &      &      &      &      &      &      &      &      &      &      & 1.08                    

                        & 1.08                                         & 1.08 \\
\bottomrule  
                                        
\end{tabular}
